Minimal Synthesis of String To String Functions From Examples

We study the problem of synthesizing string to string transformations from a set of input/output examples. The transformations we consider are expressed using deterministic finite automata (DFA) that read pairs of letters, one letter from the input and one from the output. The DFA corresponding to these transformations have additional constraints, ensuring that each input string is mapped to exactly one output string. We suggest that, given a set of input/output examples, the smallest DFA consistent with the examples is a good candidate for the transformation the user was expecting. We therefore study the problem of, given a set of examples, finding a minimal DFA consistent with the examples and satisfying the functionality and totality constraints mentioned above. We prove that, in general, this problem (the corresponding decision problem) is NP-complete. This is unlike the standard DFA minimization problem which can be solved in polynomial time. We provide several NP-hardness proofs that show the hardness of multiple (independent) variants of the problem. Finally, we propose an algorithm for finding the minimal DFA consistent with input/output examples, that uses a reduction to SMT solvers. We implemented the algorithm, and used it to evaluate the likelihood that the minimal DFA indeed corresponds to the DFA expected by the user.

==> conclusion.tex <==
% !TEX root = draft.tex

\section{Summary of the Complexity Results and Conclusion}



\input table-summary

Table~\ref{table:summary} summarizes the various complexity results 
proved in this paper.


\ctodo{As far as we know, the problem is open when the input alphabet has 
size one, i.e.~$|\Sigma| = 1$. Explain that this corresponds to finding 
an automata consistent with a finite number of examples, which is both 
thin and length-complete.}

\ctodo{Write conclusion.}


==> integers.tex <==
% !TEX root = draft.tex

\section{Adaptation to Integer Programs}
\label{section:integers}

\ctodo{Say we use the standard trick of representing numbers in binary 
and reading them simultaneously from the lsb.}
